Labelled Lambda-calculi with Explicit Copy and Erase

We present two rewriting systems that define labelled explicit substitution lambda-calculi. Our work is motivated by the close correspondence between Levy's labelled lambda-calculus and paths in proof-nets, which played an important role in the understanding of the Geometry of Interaction. The structure of the labels in Levy's labelled lambda-calculus relates to the multiplicative information of paths; the novelty of our work is that we design labelled explicit substitution calculi that also keep track of exponential information present in call-by-value and call-by-name translations of the lambda-calculus into linear logic proof-nets.

==> eptcsdata.tex <==
\providecommand{\event}{M. Florido and I. Mackie (Eds.): First International\\
Workshop on Linearity (LINEARITY 2009)}
\providecommand{\volume}{22}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{49}
\providecommand{\eid}{5}

